Leveraging Robotic Prior Tactile Exploratory Action Experiences For Learning New Objects's Physical Properties

Reusing the tactile knowledge of some previously-explored objects helps us humans to easily recognize the tactual properties of new objects. In this master thesis, we enable arobotic arm equipped with multi-modal artificial skin, like humans, to actively transfer the prior tactile exploratory action experiences when it learns the detailed physical properties of new objects. These prior tactile experiences are built when the robot applies the pressing, sliding and static contact movements on objects with different action parameters and perceives the tactile feedbacks from multiple sensory modalities. Our method was systematically evaluated by several experiments. Results show that the robot could consistently improve the discrimination accuracy by over 10% when it exploited the prior tactile knowledge compared with using no transfer method, and 25% when it used only one training sample. The results also show that the proposed method was robust against transferring irrelevant prior tactile knowledge.

==> frontmatter/declaration.tex <==
%
% File: declaration.tex
% Author: V?ctor Bre?a-Medina
% Description: Contains the declaration page
%
% UoB guidelines:
%
% Author's declaration
%
% I declare that the work in this dissertation was carried out in accordance
% with the requirements of the University's Regulations and Code of Practice
% for Research Degree Programmes and that it has not been submitted for any
% other academic award. Except where indicated by specific reference in the
% text, the work is the candidate's own work. Work done in collaboration with,
% or with the assistance of, others, is indicated as such. Any views expressed
% in the dissertation are those of the author.
%
% SIGNED: .............................................................
% DATE:..........................
%
\chapter*{Author's declaration}
\begin{quote}
I declare that the work in this master thesis was carried out in accordance with the requirements of  the University's Regulations and that it has not been submitted for any other academic award. Except where indicated by specific  reference in the text, the work is the candidate's own work. Work done in collaboration with, or with the assistance of, others, is indicated as such. Any views expressed in the thesis are those of the author.

\vspace{1.5cm}
\noindent
\hspace{-0.75cm}\textsc{SIGNED: .................................................... DATE: ..........................................}
\end{quote}
\clearpage
